Analyzing the Efficacy of an LLM-Only Approach for Image-based Document Question Answering

Recent document question answering models consist of two key components: the vision encoder, which captures layout and visual elements in images, and a Large Language Model (LLM) that helps contextualize questions to the image and supplements them with external world knowledge to generate accurate answers. However, the relative contributions of the vision encoder and the language model in these tasks remain unclear. This is especially interesting given the effectiveness of instruction-tuned LLMs, which exhibit remarkable adaptability to new tasks. To this end, we explore the following aspects in this work: (1) The efficacy of an LLM-only approach on document question answering tasks (2) strategies for serializing textual information within document images and feeding it directly to an instruction-tuned LLM, thus bypassing the need for an explicit vision encoder (3) thorough quantitative analysis on the feasibility of such an approach. Our comprehensive analysis encompasses six diverse benchmark datasets, utilizing LLMs of varying scales. Our findings reveal that a strategy exclusively reliant on the LLM yields results that are on par with or closely approach state-of-the-art performance across a range of datasets. We posit that this evaluation framework will serve as a guiding resource for selecting appropriate datasets for future research endeavors that emphasize the fundamental importance of layout and image content information.

==> tables/finetuned_slimmer.tex <==
\begin{table}
\small
  \caption{\small \textbf{Finetuned} results on four datasets (\textit{val} split) and comparisons with the state-of-the-art results from literature. All the methods in the top portion use a vision encoder and/or position information of the text in the images, whereas the bottom section only use a sequence of reading ordered text as input. The best results in each group are highlighted in bold.}
  
  %% Add DoNuT? with 143M params --> Only Test Set Numbers: 67.5 (DocVQA)
  \label{table:finetune}
  \centering
  \resizebox{0.47\textwidth}{!}
  {
    \begin{tabular}{@{}clccccc@{}}
    \toprule
    & Model            &  OCR-VQA & DocVQA & InfoVQA & TextVQA \\ 
    \midrule
    \multirow{8}{*}{\rotatebox{90}{\small With Vision Encoder}} & LaTR-B \cite{biten2021latr}   &        67.5    &     -   &      -       &       59.5  \\
    & LaTR-L  \cite{biten2021latr}     &    -     &     -   &       -          &        61.1  \\
    & Layout LMv3 \cite{huang2022layoutlmv3}     &    -     &     83.4  &            -     &   -    \\
    & DONUT  \cite{kim2022ocrfree}   & - & 67.5 & - & - \\

    & Pix2Struct-B \cite{lee2022pix2struct}  &     69.4    &    72.1    &        38.2         &   -     \\
    & Pix2Struct-L \cite{lee2022pix2struct}    &      \textbf{71.3}   &     76.6   &         40.0       &    -     \\ 
    % & LoRRA \cite{fillup} &        &    -     &     -   &            -     &    27.6     \\
    & UDOP  \cite{udop}              &    -     &  \textbf{84.7}      &        \textbf{47.4}         &     -    \\
    & PaLI \cite{chen2022pali}     &    -     &     -   &            -     &     \textbf{71.8}    \\ \midrule
    \multirow{4}{*}{\rotatebox{90}{\small Only LLM}} & FlanT5-B       &     67.2   &    69.2    &      31.7           &    54.5     \\
    & FlanT5-L       &     68.5    &   73.6    &       37.4          &     58.4    \\
    & FlanT5-XL        &     69.6    &     77.2   &         42.2        &     61.4    \\
    & FlanT5-XXL       &     \textbf{70.5}    &    \textbf{78.5}     &         \textbf{45.2}      &     \textbf{63.6}   \\
    \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/ocr_lengths.tex <==
\begin{table}
  \caption{\textbf{Median tokenized OCR length}. All results are with FlanT5-B}
  \label{table:ocr_lengths}
  \centering
    \begin{tabular}{@{}lccccc@{}}
    \toprule
      Data           & OCR-VQA & DocVQA & InfoVQA & TextVQA \\ 
    \midrule
  Before Finetune (C) & 31.0 & 375.0 & 476.0& 31.0\\
Before Finetune (I) & 34.0 & 402.0 & 645.5& 30.0\\
    Num of Correct Predictions - C & 34186 & 1963 & 451& 1780\\
     Num of Incorrect Predictions - I & 65851 & 3386 & 2350& 3220\\
        \midrule
After Finetune (C) & 32.0 & 380.0 &  478.0& 30.0\\
  After Finetune (I) & 34.0 & 423.5 & 766.0 & 31.0\\
   
        Num of Correct Predictions - C & 67216 &  3725 & 1033& 2949 \\
     Num of Incorrect Predictions - I & 32821 &  1624& 1768 & 2051\\
    \bottomrule
    \end{tabular}
\end{table}
% % Answer exists in OCR (A)
% 0.99 / 0.96
% 0.98/  0.80
% 0.92 / 0.85
% 0.87 / 0.69
% \begin{table}
%   \caption{\textbf{Impact of tokenized OCR length}. All results are on FlanT5-BASE \cite{fillup}.}
%   \label{table:readingorder}
%   \centering
%     \begin{tabular}{@{}lccccc@{}}
%     \toprule
%     Model            & FlanT5-B & FlanT5-L & FlanT5-XL & FlanT5-XXL \\ 
%     \midrule
%     Random & 52.9 & 57.2 & 60.2& 61.2\\
%     % Learned model & & & & \\
%     Standard RO & 66.6 & 71.0 & 74.6 & 77.0 \\
%     Optimal RO & \textbf{69.2} & \textbf{73.6} & \textbf{77.2} & \textbf{78.5}\\
%     \bottomrule
%     \end{tabular}
% \end{table}


==> tables/reading_order.tex <==
\begin{table}
  \caption{\textbf{Importance of reading order}. All results are on the DocVQA dataset \cite{fillup}.}
  \label{table:readingorder}
  \centering
    \begin{tabular}{@{}lccccc@{}}
    \toprule
    Model            & FlanT5-B & FlanT5-L & FlanT5-XL & FlanT5-XXL \\ 
    \midrule
    Random & 52.9 & 57.2 & 60.2& 61.2\\
    % Learned model & & & & \\
    Standard RO & 66.6 & 71.0 & 74.6 & 77.0 \\
    Raster Scan & \textbf{69.2} & \textbf{73.6} & \textbf{77.2} & \textbf{78.5}\\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/shuffle.tex <==
\begin{table}
\caption{\textbf{Performance with random reading order}. All results are for FlanT5-XXL finetuned with the given scheme for obtaining OCR context}
  \label{table:shuffle}
  \centering
    \begin{tabular}{@{}lccccc@{}}
    \toprule
    Scheme & OCR-VQA & DocVQA & InfoVQA & TextVQA \\ 
    \midrule
    Normal & 70.5 & 77.0 & 45.2 & 63.6 \\
    Random  & 63.3 & 61.2 & 25.07 & 53.9\\
    % % Learned model & & & & \\
    % Standard RO & 66.6 & 71.0 & 74.6 & 77.0 \\
    % Raster Scan & \textbf{69.2} & \textbf{73.6} & \textbf{77.2} & \textbf{78.5}\\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/structured.tex <==
\begin{table}[h!]
  \caption{Finetuned FlanT5-L on Structure Extraction Task (OCR-VQA). }
  
  \label{table:structured}
  \centering
    \begin{tabular}{@{}clccccc@{}}
    \toprule
    &      Metric      & Titles & Authors & Genre \\ 
    \midrule
    & Exact Match     &     41.6    &   67.2     &       70.8   \\
    & ANLS & 71.2 & 75.8 & 70.9 \\
    \bottomrule
    \end{tabular}
\end{table}

% CKPT: 1219000
% Titles:  (0.41597608884712656, 0.7115402465702071)
% Authors:  (0.6719413816887752, 0.7579963739176375)
% Genres:  (0.7080980037386168, 0.7086603830100646)
